Twig: Parallel and Memory-Efficient Tree Speculative Decoding for Hybrid-Attention LLMs

Emerging LLMs increasingly interleave full attention with recurrent linear attention to reduce long-context serving costs. Tree speculative decoding could further accelerate these hybrid models, but recurrent linear-attention layers carry parent-dependent states. Existing engines therefore verify proposal trees sequentially and snapshot the full state per node, causing latency and memory to grow with tree and batch sizes. We present Twig, a kernel--runtime co-design for tree speculative decoding of hybrid LLMs. Twig derives a tree-structured factorization of the linear-attention recurrence and realizes it with a resource-efficient GPU kernel that verifies all nodes in parallel, accelerating linear-attention tree verification by 3.4--7.7$\times$. It losslessly represents speculative state updates as token-level factors and reconstructs only the accepted state, reducing transient state memory by 82--99$\times$ and freeing GPU memory for KV caches. We integrate Twig into SGLang, a widely deployed production LLM serving engine, and further optimize its runtime through batch-wide verification budgeting. Across four models, two GPU platforms, and diverse datasets, Twig achieves up to $4.72\times$ the offline decode throughput of autoregressive decoding and up to $2.03\times$ that of the strongest tree-speculative baseline. Under online agent workloads, Twig reduces TTFT and TPOT by up to $67.6\%$ and $49.9\%$, respectively, over the strongest tree-speculative baseline.

==> macros.tex <==
% Twig-specific notation and formatting commands.
% Revision categories: common concerns and Reviewers A--F.
% The switch is configured in main.tex before this file is loaded.
\ifrevisioncolors
  \RequirePackage[authormarkup=none]{changes}
\definecolor{cCommon}{HTML}{FF0000}
\definecolor{cA}{HTML}{0072B2}
\definecolor{cB}{HTML}{228833}
\definecolor{cC}{HTML}{AA3377}
\definecolor{cD}{HTML}{996600}
\definecolor{cE}{HTML}{00838F}
\definecolor{cF}{HTML}{663399}
\definechangesauthor[color=cCommon]{common}
\definechangesauthor[color=cA]{A}
\definechangesauthor[color=cB]{B}
\definechangesauthor[color=cC]{C}
\definechangesauthor[color=cD]{D}
\definechangesauthor[color=cE]{E}
\definechangesauthor[color=cF]{F}
\RequirePackage{marginnote}
% Optional question IDs use changes comments, with no automatic counters.
% Non-floating margin notes also work inside figure and table captions.
\setcommentmarkup{%
  \ifrevisionlabels
    \begingroup
      \setlength{\marginparwidth}{30pt}%
      \setlength{\marginparsep}{4pt}%
      \marginnote{\scriptsize\sffamily\bfseries\color{authorcolor}#1}%
    \endgroup
  \fi}
% Show only revised wording, not deleted text or replacement strikeouts.
\setdeletedmarkup{}
\DeclareRobustCommand{\cq}[2][]{\added[id=common,comment={#1}]{#2}}
\DeclareRobustCommand{\ra}[2][]{\added[id=A,comment={#1}]{#2}}
\DeclareRobustCommand{\rb}[2][]{\added[id=B,comment={#1}]{#2}}
\DeclareRobustCommand{\rc}[2][]{\added[id=C,comment={#1}]{#2}}
\DeclareRobustCommand{\rd}[2][]{\added[id=D,comment={#1}]{#2}}
\DeclareRobustCommand{\re}[2][]{\added[id=E,comment={#1}]{#2}}
\DeclareRobustCommand{\rf}[2][]{\added[id=F,comment={#1}]{#2}}
\else
% Print revised text directly in the public version.
\DeclareRobustCommand{\cq}[2][]{#2}
\DeclareRobustCommand{\ra}[2][]{#2}
\DeclareRobustCommand{\rb}[2][]{#2}
\DeclareRobustCommand{\rc}[2][]{#2}
\DeclareRobustCommand{\rd}[2][]{#2}
\DeclareRobustCommand{\re}[2][]{#2}
\DeclareRobustCommand{\rf}[2][]{#2}
\fi
% Keep color commands out of PDF bookmarks.
\NewExpandableDocumentCommand{\revisionpdftext}{O{} m}{#2}
\pdfstringdefDisableCommands{%
  \let\cq\revisionpdftext\let\ra\revisionpdftext%
  \let\rb\revisionpdftext\let\rc\revisionpdftext%
  \let\rd\revisionpdftext\let\re\revisionpdftext%
  \let\rf\revisionpdftext}

\newtheoremstyle{compactplain}
  {3.5pt plus 1pt minus 1pt}
  {3.5pt plus 1pt minus 1pt}
  {\itshape}
  {}
  {\bfseries}
  {.}
  {0.5em}
  {}
\theoremstyle{compactplain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}

\makeatletter
\renewenvironment{proof}[1][\proofname]{\par
  \pushQED{\qed}%
  \normalfont \topsep3\p@\@plus1\p@\@minus1\p@\relax
  \trivlist
  \item[\hskip\labelsep\itshape #1\@addpunct{.}]\ignorespaces
}{%
  \popQED\endtrivlist\@endpefalse
}
\makeatother

\newenvironment{compactequation}{%
  \setlength{\abovedisplayskip}{1.1ex plus 0.75pt minus 0.4pt}%
  \setlength{\belowdisplayskip}{1.1ex plus 0.75pt minus 0.4pt}%
  \setlength{\abovedisplayshortskip}{0.25pt plus 1pt}%
  \setlength{\belowdisplayshortskip}{1.1ex plus 0.75pt minus 0.4pt}%
  \begin{equation}%
}{%
  \end{equation}%
}

\newcommand{\Anc}{\mathcal{A}}
\newcommand{\Spre}{S_{\mathrm{pre}}}
\newcommand{\ind}{\mathbf{1}}
\newcommand{\sys}{\sysname\xspace}

\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\figsref}[2]{Figs.~\ref{#1} and~\ref{#2}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\eqnref}[1]{Eq.~\eqref{#1}}
\newcommand{\secref}[1]{\S~\ref{#1}}
\newcommand{\secrefs}[2]{Sections~\ref{#1}--\ref{#2}}

\newcommand{\runinhead}[1]{%
  \par\vspace{1.325pt}\noindent\textbf{#1}\enspace\ignorespaces}

\setlength{\textfloatsep}
  {1.4\baselineskip plus 0.1\baselineskip minus 0.2\baselineskip}
\setlength{\dbltextfloatsep}
  {1.4\baselineskip plus 0.1\baselineskip minus 0.2\baselineskip}

